Lifting Weak Supervision To Structured Prediction

Weak supervision (WS) is a rich set of techniques that produce pseudolabels by aggregating easily obtained but potentially noisy label estimates from a variety of sources. WS is theoretically well understood for binary classification, where simple approaches enable consistent estimation of pseudolabel noise rates. Using this result, it has been shown that downstream models trained on the pseudolabels have generalization guarantees nearly identical to those trained on clean labels. While this is exciting, users often wish to use WS for structured prediction, where the output space consists of more than a binary or multi-class label set: e.g. rankings, graphs, manifolds, and more. Do the favorable theoretical properties of WS for binary classification lift to this setting? We answer this question in the affirmative for a wide range of scenarios. For labels taking values in a finite metric space, we introduce techniques new to weak supervision based on pseudo-Euclidean embeddings and tensor decompositions, providing a nearly-consistent noise rate estimator. For labels in constant-curvature Riemannian manifolds, we introduce new invariants that also yield consistent noise rate estimation. In both cases, when using the resulting pseudolabels in concert with a flexible downstream model, we obtain generalization guarantees nearly identical to those for models trained on clean data. Several of our results, which can be viewed as robustness guarantees in structured prediction with noisy labels, may be of independent interest. Empirical evaluation validates our claims and shows the merits of the proposed method.

==> sections/checklist.tex <==
\section*{Checklist}
%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:

%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

%\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them? \answerYes{}
    
    \item Did you state the full set of assumptions of all theoretical results? \answerYes{}
   \item Did you include complete proofs of all theoretical results?
    \answerYes{See appendix} 
\end{enumerate}




==> sections/tools.tex <==
Next we introduce three tools that we use for our approach. The first pair are required for the finite metric space case, while the latter is used for the continuous-space case.

\subsection{Embedding in Pseudo-Euclidean Spaces}
Working directly with the label space $\cY$ is challenging and it limits the set of tools we can use. A common way to get around this problem is to embed the points of $\cY$  into a suitable vector space. Perhaps the most standard approach to producing metric embeddings is via multi-dimensional scaling (MDS) \cite{KruskalWish1978}. The downside of MDS is that only some metric spaces embed (isometrically) into Euclidean space. In particular, it is necessary that the square distance matrix $\bD$ is positive semi-definite. 

A simple and elegant way to overcome this difficulty is to instead use \emph{pseudo-Euclidean} spaces for embeddings. These pseudo-spaces do not require a p.s.d. inner product. As an outcome, any finite metric space can be embedded into a pseudo-Euclidean space with \emph{no distortion} \cite{goldfarb85psuedo}. Without going into the technicalities of pseudo-Euclidean spaces here we state some relevant facts that will be useful later. More in-depth background on these spaces is provided in the appendix.

\textbf{Pseudo-Euclidean Spaces:}
A vector $\bu$ in a pseudo-Euclidean space $\psR$ has two parts $\bu^+ \in \R^{d^+}$ and $\bu^- \in \R^{d^-}$, where $\R^{d^+},\R^{d^-}$ are Euclidean spaces of dimension $d^+$ and $d^-$ respectively.  The dot product and the squared distance between any two vectors $\bu,\bv$ in a pseudo-Euclidean space $\psR$ are expressed as,
\begin{equation}
    \langle \bu, \bv\rangle_{\phi} = \langle \bu^+,\bv^+ \rangle - \langle \bu^-,\bv^- \rangle \qquad   d^2_{\phi}(\bu,\bv) =  ||\bu^{+}-\bv^{+}||_2^2 - ||\bu^{-}-\bv^{-}||_2^2   %=\langle \bu, \bM_{\phi}\bv     \rangle 
\end{equation}
%\begin{equation}
 %   d^2_{\phi}(\bu,\bv) =  ||\bu^{+}-\bv^{+}||_2^2 - ||\bu^{-}-\bv^{-}||_2^2 =  \langle \bu -\bv , \bM_\phi (\bu-\bv) \rangle
%\end{equation}
%Here the matrix $\bM_{\phi} = \begin{pmatrix} \bI_{d^+} & \b0 \\ \b0 & \bI_{d^-} \end{pmatrix}$  is associated with the pseudo-Euclidean space $\psR$ and $\bI_{d^+}, \bI_{d^-}$ are the identity matrices of dimensions $d^{+},d^{-}$ respectively. It is important to note that despite the distance function having negative terms, the distances will always remain non-negative.
\textbf{Pseudo-Euclidean Embeddings:} 
Let $g:\cY\mapsto \R^{(d^+,d^-)}$ be the isometric embedding function and denote the outputs of the embedding function as $\blm_a = g(\lambda_a)$ and $\by = g(y)$. Also let $\Y  = \{\by: \by=g(y) \,\forall y\in \cY \}\subset \R^{(d^+,d^-)}$ be the collection of embeddings of all objects in $\cY$.  Note since the embedding function is a bijection so  $|\Y| = |\cY|$ and these sets are finite.
Since $g$ gives isometric embeddings in the pseudo-Euclidean space, the distance between any $\lambda_a$ and $y$ in the pseudo-metric space is equal to the distance between their vector representations in the pseudo-Euclidean space i.e. $d_\cY(\lambda_a,y) = d_\phi(\blm_a,\by)$ \cite{goldfarb85psuedo}.


\subsection{Tensor Decompositions}
Tensor decompositions \cite{anandkumar2014tensor, anandkumar2014sample} are a powerful tool used to solve a variety of latent-variable problems, including topic models, multi-view models, hidden Markov models (HMMs), and mixtures of Gaussians. Such models have not been applied to the weak supervision setting; we shall see that they permit nearly consistent estimation of our label model's parameters.

